LM-GAN: A Photorealistic All-Weather Parametric Sky Model

We present LM-GAN, an HDR sky model that generates photorealistic environment maps with weathered skies. Our sky model retains the flexibility of traditional parametric models and enables the reproduction of photorealistic all-weather skies with visual diversity in cloud formations. This is achieved with flexible and intuitive user controls for parameters, including sun position, sky color, and atmospheric turbidity. Our method is trained directly from inputs fitted to real HDR skies, learning both to preserve the input's illumination and correlate it to the real reference's atmospheric components in an end-to-end manner. Our main contributions are a generative model trained on both sky appearance and scene rendering losses, as well as a novel sky-parameter fitting algorithm. We demonstrate that our fitting algorithm surpasses existing approaches in both accuracy and sky fidelity, and also provide quantitative and qualitative analyses, demonstrating LM-GAN's ability to match parametric input to photorealistic all-weather skies. The generated HDR environment maps are ready to use in 3D rendering engines and can be applied to a wide range of image-based lighting applications.

==> figures/format_info/format_info.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/format_info/format.pdf}
    \caption{Properly capturing the full high dynamic range (HDR) of outdoor lighting is of paramount importance. (a) an HDR equirectangular image of the sky shown at three different exposures (1, 1/10, 1/100) illustrates that the sun is orders of magnitude brighter than the sky (see profile in the top row). Accordingly, relighting a scene with an LDR sky (b) fails to reproduce proper HDR lighting effects (c).}
    \label{fig:hdrvsldr}
\end{figure}

==> figures/percentile_plots/overall_plots.tex <==
\begin{figure}[htbp]
    \centering
    \footnotesize
    \begin{tabular}{c}
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_rmse.pdf} \\
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_si_rmse.pdf} \\
    (a) RMSE (top) and si-RMSE (bottom) for the texture \\
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_ltm_gt_rmse.pdf} \\
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_ltm_gt_si_rmse.pdf} \\
    (b) RMSE (top) and si-RMSE (bottom) for the lighting (compared to reference)\\
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_ltm_lm_rmse.pdf} \\
    \includegraphics[width=\linewidth,trim={0 0.5cm 0 0.5cm},clip]{figures/percentile_plots/plots/percentiles_ltm_lm_si_rmse.pdf} \\
    (c) RMSE (top) and si-RMSE (bottom) for the lighting (compared to the input)
    \end{tabular}
    \caption{Distribution of RMSE and si-RMSE errors for the different metrics. From top to bottom: texture, lighting (compared to reference), and lighting (compared to the input). Our approach provides lower error distributions in all cases.}
    \label{fig:scores}
\end{figure}
